Vulnerability of D2D Communications from Interconnected Social Networks

In this paper, we study how rumors in Online Social Networks (OSNs) may impact the performance of device-to-device (D2D) communication. As D2D is a new technology, people may choose not to use it when believed in rumors of its negative impacts. Thus, the cellular network with underlaying D2D is vulnerable to OSNs as rumors in OSNs may decrement the throughput of the cellular network in popular content delivery scenarios. To analyze the vulnerability, we introduce the problem of finding the most critical nodes in the OSN such that the throughput of a content delivery scenario is minimized when a rumor starts from those nodes. We then propose an efficient solution to the critical nodes detection problem. The severity of such vulnerability is supported by extensive experiments in various simulation settings, from which we observe up to $40\%$ reduction in network throughput.

==> vulnerability-d2d-communications (1)/experiment.tex <==

\section{Experiments}\label{sec:experiment}

In this section, we evaluate how cellular network performance can be impacted when the critical nodes in the OSN propagates the rumor. In the following, we first discuss the setup for the experiments in Section \ref{ssec:setup}. In Section \ref{ssec:misinfo}, we measure the vulnerability of the cellular network. Then we consider how the actions of the users and the BS can reduce the vulnerability in Section \ref{ssec:awareness} and \ref{ssec: retention}, respectively.

\subsection{Setup}\label{ssec:setup} 

\textbf{Cellular Network.} As the real data sets are limited due to our requirements, we choose to use synthetic data for the cellular network. In a square $50$m by $50$m area, we generate $50$ data requesters at random locations. Further, we select $30$ of them to be in D2D mode and the other $20$ remain in cellular mode. To enable D2D communication, we also generate $60$ D2D relay devices at random locations within the area.  All the wireless parameters are summarized in Table~\ref{table:wirelessparam}. 

%the impact of the attacks on cellular networks with moderate number of data requesters and large number of stable D2D links. However, the real-world data sets are limited due to our requirements. As the purpose of the paper is to illustrate the severeness of the attacks and cast light upon the new threats, simulated data suffices. Therefore, we choose to use synthetic data for the cellular network. In a square $50$m by $50$m area, we generate $50$ data requesters at random locations. Further, we select $30$ data requesters to be in D2D mode and the other $20$ remain in cellular mode. To enable D2D communication, we also generate $60$ D2D relay devices at random locations within the area.  All the wireless parameters are summarized in Table \ref{table:wirelessparam}. 

\textbf{OSN.} To model information propagation in the OSN, we use real-world Facebook network topology from \cite{snap}. The Facebook data consists of 4039 users and 88234 social network interactions between the users \cite{mcauley2012learning}. The influence between a pair of users was assigned randomly from a uniform distribution.
\begin{table}
	\caption{Wireless Network Parameters} 
	\begin{tabular}{|c|c|}
		\hline Notation & Description \\
        \hline Cell dimension & $50$ x $50$ $m^2$ \\ 
        \hline BS position  & Lower left corner \\ 
        \hline Network bandwidth & $0.1$ MHz \\ 
		\hline Channel Model & Multipath Rayleigh
fading \\ 
        \hline Path Loss Exponent & $3$ \\ 
        \hline Noise spectral density & $-174$ dBm/Hz \\ 
		\hline BS transmit power& $100$ W \\ 
		\hline D2D transmit power & $10$ W \\ 
        \hline D2D distance & $15$ m\\
		\hline
	\end{tabular}

	\label{table:wirelessparam}
\end{table}

\textbf{Interdependency.} For the interconnection between the two networks, we consider two scenarios, namely a stadium scenario and a shopping mall scenario. In the stadium scenario, the owners of the devices are not very likely to be socially connected. In the shopping mall scenario, however, as the shoppers normally resides closer than the game goers, the owners of the devices are more likely to be connected in the OSN, compared with the stadium scenario. 

We use the following procedure to create the interconnections. For each D2D node $i\in V^d$, we construct link $e^{vi}$ between $i$ and a uniformly randomly chosen user $v\in V^s$ from the OSN. Once $e^{vi}$ is constructed, with probability $p_1$, we uniformly randomly choose a neighbor $i'$ of $i$ and a neighbor $v'$ of $v$ and construct link $e^{v'i'}$. With probability $p_2$, we construct link $e^{\bar{v}\bar{i}}$ for a random neighbor $\bar{i}$ of $i'$ and a random neighbor $\bar{v}$ of $v'$, when $e^{v'i'}$ is constructed. In order to differentiate the different level of social connections among users in the cell area, we apply higher $p_1,p_2$ values for the shopping mall scenario. In our experiments we have set $p_1=0.7$ and $p_2=0.4$ for the stadium scenario, and $p_1=0.9$ and $p_2=0.6$ for the shopping mall scenario.

\textbf{Algorithms.} To illustrate the efficacy of our proposed method RCF, especially the criticalness evaluation scheme, we compare RCF with two approaches. The first approach uses degree centrality as criticalness values and runs the same targeted IM algorithm embedded in RCF to obtain the critical nodes in the OSN. The second approach, as a baseline, randomly assigns criticalness values to guide critical nodes selection in the OSN. 
%For the D2D network, we have considered a fully occupied stadium during a game event. We have shown the impact of rumor in social network on the D2D by further considering a square $50$m x $50$m area segment of the stadium which contains 5251 viewers. We randomly assigned 18 users as the set of cellular users $V^c$ and 27 users as D2D receivers $R^d$ seeking for a particular content. We assumed the BS is at the bottom of the leftmost corner of the considered area. We have set the number of relay devices $|V^r|=63$.

%We also consider another scenario where the cell is located in a residential area. The users who are within maximum D2D distance form a D2D pair. For this residential network, We consider the similar number of cellular and D2D users and receivers and also same wireless network parameters that we considered for the stadium. However, the users of this residential area are likely to have strong social relationship between themselves as compared to random users sitting next to each other in stadium. As a result, users forming the D2D network in the residential area are likely to be impacted more by the misinformation propagation in the corresponding social network. We report relevant results pertaining to this phenomenon later in this section. 



\subsection{Vulnerability of the Cellular Network}\label{ssec:misinfo}
In this section, we study how vulnerable the cellular network is to rumors in the OSN, in terms of throughput reduction. Also, we demonstrate that social connectivity of the nodes in the cellular network can impact the vulnerability. Additionally, we explore another dimension of vulnerability: how much bandwidth is necessary to bring the throughput back to the original value. 
\begin{figure}[!ht] \centering
\caption{Throughput Reduction}
\subfloat[Stadium Scenario]{
 	\includegraphics[width=0.49\linewidth]{Figures/througput.pdf}
 	%\caption{D2D communications offload data from BS.}
 	\label{fig:thr}}
\subfloat[Shopping Mall Scenario]{
 	\includegraphics[width=0.49\linewidth]{Figures/througput_res.pdf}
 	%\caption{D2D communications are not possible after users being affected by misinformation.}
 	\label{fig:user_affected}}

    \label{fig:throughputdec}
 \end{figure}
 
We first observe how the throughput can be impacted with varying seed set size of spreading rumors in the OSN. In Figure \ref{fig:throughputdec}, for both scenarios, the throughput of the cellular network experiences substantial decreases after the rumor propagation. The decrements are higher with increasing number of seeds (i.e. critical nodes). With RCF, the damage to throughput is severer than other approaches, which means that RCF can better reveal the critical nodes. The gap between RCF and the other methods increases significantly as more seed nodes can be selected. In Figure \ref{fig:thr}, the throughput drops $40\%$ when $10$ critical nodes outputted by RCF are used as seeds of rumor. It is worth noticing that even the random approach can lead to noticeable decrease in throughput. Therefore, the interdependent cellular/social networks is vulnerable not only to rumors that are intentionally spread, but also to those that are randomly originated.



\begin{figure*}[!ht] 
\begin{minipage}[t]{0.31\linewidth}
\centering
\includegraphics[width=1\linewidth]{Figures/througput_decrease_rate.pdf}
\caption{Stadium versus Shopping Mall: higher social connectivity results in faster drop of throughput}
\label{fig:res}
\end{minipage}
\hfill
\begin{minipage}[t]{0.31\linewidth}
\centering
 	\includegraphics[width=1\linewidth]{Figures/extra_bw.pdf}
 	\caption{Extra bandwidth requirement for the stadium scenario}
 	\label{fig:new_resource}
\end{minipage}
\hfill
\begin{minipage}[t]{0.31\linewidth}
\centering
 	\includegraphics[width=1\linewidth]{Figures/ua_k10.pdf}
 	\caption{Impact of user awareness on network throughput (adversary's budget is 10)}
 	\label{fig:ua_k10}
 \end{minipage}

\end{figure*}

Next, we examine how social connectivity impacts the throughput. In theory, in a network with higher level of social connections, rumors can cause larger influence than a network with less social connections, with the same seed set size. Therefore, the cellular network can be more vulnerable when the interdependent OSN is more densely connected. 

The result depicted in Figure \ref{fig:res} supports the analysis. At each seed set size,  we calculate the relative throughput decrease $Q_k$ for different scenarios. Denote the throughput after rumor propagation with $k$ seed nodes as $T_k$, we define $Q_k=\frac{T_0-T_k}{T_0}\times 100\%$. 

As can be seen from Figure \ref{fig:res}, $Q_k$ for the shopping mall scenario increases faster in most of the cases, which demonstrates that the social connections actually aid the rumor propagation, as well as increase the vulnerability. The slow increase in $Q_k$ for the shopping mall scenario after seed set size $8$ can be interpreted as a saturation case, that all D2D users are already influenced and the throughput cannot be further decreased. It explains why $Q_k$ of the stadium scenario surpasses that of the shopping mall scenario after seed set size $8$.

Then, we show in Figure \ref{fig:new_resource} the additional bandwidth cost requirement that arises from increasing the throughput to the level before rumor propagation. Consistent with our previous findings, the critical nodes found by RCF result in the largest bandwidth requirement and thus exerts the highest pressure to the BS. After the rumor propagation, the extra bandwidth required can be up to $1400$Hz. When a BS runs out of its own bandwidth and fails to supply the additional bandwidth, the throughput will be decreased drastically and the data requesters can experience a low data rate, which is not preferable. However, supply the extra requirement can be costly and thus a heavy burden to the BSs. This phenomenon emphasizes how vulnerable the cellular network can be, from another direction.  

\subsection{Reduce Vulnerability from the OSN}\label{ssec:awareness}
In this section, we study how users' actions can help in reducing the vulnerability of the cellular network. In OSNs, not all users are equally sensitive to rumors of D2D communication. Users having larger exposure to related knowledge are likely to identify the rumors and remain uninfluenced. So, they are not likely to opt out using D2D nor spread the rumor. In contrast, the users with limited knowledge to D2D are susceptible to rumors and are much more likely to opt out using D2D.  

To quantitatively describe the users' knowledge to D2D, we use the term "User Awareness" (UA) which ranges from $0.0$ to $1.0$ with $1.0$ means most aware of D2D related rumors. UA is in effect in the IC model in the following way. Denote the awareness for user $v$ as $W_v$. In the original IC model, node $u$ can influence node $v$ with probability $p_{uv}$. With UA, the probability is modified to $p_{uv}\times(1-W_v)$. Therefore, the most aware users ($W_v=1$) can never be influenced. Clearly, when users become more aware of the rumors, the rumor propagation will be limited and the vulnerability of the cellular network to the rumors will be reduced. 

In this experiment, we fix the number of seed nodes at $10$ and vary UA values between $0$ and $1$ in the stadium scenario. As the results for the shopping mall scenario have the similar trend, we choose not to include them for conciseness. Notice that we set the UA values equally for all nodes. Such a case can describe the situation in which the general public is educated about D2D and the individuals have similar awareness. Figure \ref{fig:ua_k10} clearly illustrates the trend that when the user are more aware, the cellular network is less vulnerable in terms of throughput. For the degree based and random methods, the throughput recovered linearly with respect to the increase of UA. However, the seed nodes selected by RCF are "resistant" to UA. When the UA value is $0.2$, the throughput after the RCF based rumor propagation only increased by $5\%$ compared with the case without UA. This experiment illustrates that the cellular network can still be vulnerable in the worst case, even if users start to be aware of the rumors.   

To have a thorough understanding of UA, we now present the network throughput achieved by RCF for different values of user awareness values under various seed set size. Figure \ref{fig:heatmap} is the heat map representing the impact of user awareness and the number of critical nodes on the network throughput. The throughput is depicted by the RGB colors. As the throughput value gets higher, the color becomes lighter in the heat map. From Figure \ref{fig:hm}, we can see that the color is the lightest, i.e. the throughput is the highest, in the top left corner where the number of critical nodes is the least and the users are the most aware. 

\begin{figure*}[!htbp]
  \centering
\begin{minipage}[c]{0.66\textwidth}
\centering
\subfloat[][The Heat Map]{\includegraphics[width=0.49\textwidth]{Figures/heatmap_ua_k.pdf}\label{fig:hm}}
~
\subfloat[][A snap shot from Figure \subref{fig:hm}: Effect of the seed set size on the throughput.]{\includegraphics[width=0.49\textwidth]{Figures/hm_snapshot.pdf}\label{fig:snap_shot}}
~

\caption{\label{fig:heatmap} Impact of user awareness on network throughput}
\end{minipage}%
\hfill
\begin{minipage}[c]{0.33\textwidth}
\centering
\includegraphics[width=1\textwidth]{Figures/bs_protect_gain.pdf}

\caption{BS incentivizes devices to block impact from rumors.\label{fig:bs_protect}}
\end{minipage}

\end{figure*}


Sample horizontal and vertical stripes are taken in the heat map and plotted in Figure \ref{fig:snap_shot}. The throughputs are shown for four different user awareness levels (1.0, 0.4, 0.2, 0.0).
As users become more prone to rumors, which is captured by smaller user awareness values, the network throughput decreases for fixed seed set size. On the other hand, when the number of seed users increases, the throughput decreases for a given user awareness. 




\subsection{Reduce Vulnerability from the Cellular Network}\label{ssec: retention}
In Section \ref{ssec:awareness}, we demonstrate that the vulnerability can be reduced when the users can identify rumors about D2D and thus limit rumor propagation in the OSN. However, improve awareness for the general public may take time. In the meantime, the BS is responsible to ensure the usual network operation and continue to offer the best service. In this section, we discuss how the vulnerability can be reduced from the cellular network. To this end, the BS can identify the critical users to the D2D communication and incentivize them to stay using D2D. Using the same criticalness evaluation scheme, the BS can rank the devices based on their criticalness values. Once the top-ranked devices are identified, the BS offers those devices incentive to keep them in the cellular network. We now investigate how network throughput will change when the critical users are retained.

Figure \ref{fig:bs_protect} expresses the scenario where BS has a budget to incentivize the devices in the cellular network. In this experiment, we again use the stadium scenario only for conciseness and fix the number of critical nodes to $10$. We measure the performance of the incentive based approach in terms of throughput gain $G_l$ when the BS has budget $l$. Denote $T_{10}^{l}$ as the throughput calculated by RCF in the situation where the number of critical nodes is $10$ and the BS has budget of $l$. Define $G_l=\frac{G_l-T_{10}^{l}}{T_{10}^{l}}$, 
we can observe that the more budget the BS has, the larger throughput gain it achieves. Interestingly, this critical user retention scheme is much more effective against RCF compared with the other two approaches for critical nodes identification. The throughput gain is over $50\%$ with BS budget of $10$. This result suggests that incentives can be effective for reducing the vulnerability of the cellular network.


